pplacer: linear time maximum-likelihood and Bayesian phylogenetic placement of sequences onto a fixed reference tree

Likelihood-based phylogenetic inference is generally considered to be the most reliable classification method for unknown sequences. However, traditional likelihood-based phylogenetic methods cannot be applied to large volumes of short reads from next-generation sequencing due to computational complexity issues and lack of phylogenetic signal. "Phylogenetic placement," where a reference tree is fixed and the unknown query sequences are placed onto the tree via a reference alignment, is a way to bring the inferential power of likelihood-based approaches to large data sets. This paper introduces pplacer, a software package for phylogenetic placement and subsequent visualization. The algorithm can place twenty thousand short reads on a reference tree of one thousand taxa per hour per processor, has essentially linear time and memory complexity in the number of reference taxa, and is easy to run in parallel. Pplacer features calculation of the posterior probability of a placement on an edge, which is a statistically rigorous way of quantifying uncertainty on an edge-by-edge basis. It also can inform the user of the positional uncertainty for query sequences by calculating expected distance between placement locations, which is crucial in the estimation of uncertainty with a well-sampled reference tree. The software provides visualizations using branch thickness and color to represent number of placements and their uncertainty. A simulation study using reads generated from 631 COG alignments shows a high level of accuracy for phylogenetic placement over a wide range of alignment diversity, and the power of edge uncertainty estimates to measure placement confidence. Pplacer enables efficient phylogenetic placement and subsequent visualization, making likelihood-based phylogenetics methodology practical for large collections of reads; it is available as source code, binaries, and a web service.

==> trash.tex <==
\subsection*{Confidence score comparison: mean of 34aa read length}
\includegraphics[width= 5.5in]{/home/matsen/pplacer/simulations/accuracy/OSCsim2short.pdf}

The mean and standard deviation of error scores in the simulations plotted according to confidence score. 
The figure legends and read length distribution is as in Table~\tabCOG.
The fact that each of the lines in this plot trend downward indicates that the confidence score we selected does a good job of predicting the accuracy of the placement. 
For such short sequences it appears from this plot that one needs to have a confidence score of over 0.75 to expect to have a topological error of less than one.


\subsection*{Confidence score comparison: mean of 85aa read length}
\includegraphics[width= 5.5in]{/home/matsen/pplacer/simulations/accuracy/OSCsim2.pdf}

The mean and standard deviation of error scores in the simulations plotted according to confidence score. 
The figure legends and read length distribution is as in Table~\tabOSCshort.
Again, it appears that in this case the confidence score does a good job of predicting the accuracy of the placement.
For sequences of this length it appears from this plot that one needs to have a confidence score of about 0.5 to expect to have a topological error of less than one.



\subsection*{Comparison to BLAST and MEGAN}

The previous simulations show that the \pplacer\ core algorithm is equal to or better than the phylogenetic methods developed thus far in the literature.
However, one might ask how it compares against methods which are not explicitly phylogenetic in nature.
Perhaps the most commonly used way of analyzing metagenomes is via a BLAST sequence similarity search \cite{altschulEaBLAST90}.
It appears that the second most commonly used method is the MEtaGenome ANalysis (MEGAN) software of Daniel Huson and collaborators \cite{husonEaMEGAN07}, which combines taxonomic and sequence similarity approaches.

In order to compare our methods to MEGAN, we implemented the same MEGAN algorithm except that we used our reference tree in place of the NCBI taxonomy, which is how MEGAN was originally conceived.
We ran this algorithm on the simulated fragments from the previously-described fragment simulation experiment with various values of the ``top-percent'' filter, which is a user-supplied parameter that determines how deeply MEGAN puts the fragment in the tree. 
The guidelines in their paper are to use top-percent filters in the 10-20\% range, and so we ran our MEGAN implementation with this parameter set at 10, 15, and 20\%.
In addition, we investigated the placement of the best blast hit, and the \pplacer\ ML placement.
We then calculated the same topological error for each one of these methods on the same simulated fragments of mean length 85aa as before.
Before discussing the results, we would like to acknowledge that this is not in some sense a fair comparison: we are using a phylogenetically-derived error metric to score an explicitly phylogenetic algorithm (ours) against ones which are not completely phylogenetic in nature.
Nevertheless, the focus of this paper is on the best way to derive phylogenetic placements from short sequences, and thus we feel that it is important to compare our method to other popular methods which might be used to accomplish this task.

As shown in Table~XXX, \pplacer\ compares favorably to MEGAN and best blast hit analysis.




\subsection*{Table 3 - Comparison of \pplacer\ to Best Blast Hit and MEGAN}

\begin{tabular}{l|lllll}
        & 	 & 	 & \multicolumn{3}{c}{MEGAN} \\
\cline{4-6}
error   & \pplacer & BBH & 10 \% & 15 \% & 20 \% \\ 
\hline
0       & 233   & 104   & 78    & 58    & 41    \\ 
1       & 89    & 199   & 177   & 152   & 120   \\ 
2       & 22    & 11    & 55    & 66    & 79    \\ 
3       & 6     & 16    & 27    & 48    & 56    \\ 
4       & 6     & 9     & 15    & 26    & 39    \\ 
5       & 3     & 20    & 3     & 7     & 18    \\ 
6       & 0     & 0     & 2     & 1     & 5     \\ 
7       & 0     & 0     & 0     & 0     & 0     \\ 
8       & 0     & 0     & 1     & 1     & 1     \\ 
9       & 0     & 0     & 0     & 0     & 0     \\ 
\end{tabular}

The frequency of various errors for \pplacer, best blast hit, and MEGAN in a format similar to that of Tables~1 and 2. 
The percentages in the MEGAN columns are the ``top-percent'' filter, which determines the depth
In this simulation, \pplacer\ appears to outperform both best blast hit and MEGAN.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               %%
%% Additional Files              %%
%%                               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


On the methodological front, it would be interesting to investigate if a combination of HMMER E-values and phylogenetic confidence scores can be used to further improve accuracy estimation.
Another interesting issue is how one would extend the framework of this paper to several alternate reference trees.
\Pplacer can run three possible variants of phylogenetic analysis: (1) posterior probability, (2) maximum likelihood with constrained topology and branch length of the phylogenetic tree, (3) maximum likelihood with constrained topology only, and simulations were run in each of these modes for comparison.  
As described in our Methods section, we use Bayesian posterior probability and the likelihood weight distribution in order to score the placement of the fragments in the phylogenetic tree; the highest value of these quantities across different placements in the tree will be called the ``best confidence score'' (BCS).
As described in our Methods section, we use Bayesian posterior probability and the likelihood weight distribution in order to score the placement of the fragments in the phylogenetic tree; the highest value of these quantities across different placements in the tree will be called the ``best confidence score'' (BCS).
Thus, one may expect that if the confidence score is low, then we may feel more confident in the placement than if the confidence score is high.
However, there is no formal statistical methodology for establish how accurate a given placement to be if it has a given confidence score.
Thus, in order to establish the relationship between confidence and accuracy, as well as the accuracy of our algorithm, we have implemented a large-scale fragment simulation pipeline which can be used on any alignment and reference tree.

This pipeline can be used on any alignment and reference tree.

We have shown relevant plots in Figures~xxx and xxx. 
As the general trend of the curves is in a downward direction, placements with higher confidence score have lower error; thus the confidence scores do tell us something useful about the accuracy of a placement. 
All three methods appear to do a good job of estimating confidence. 
In the shorter (mean 34 amino acid) version of our simulations, a confidence score of above 0.75 seems to be the choice if one is interested in getting placements with average error less than one, whereas for the longer (mean 85 amino acid) simulations an appropriate confidence score cutoff would be around 0.5.

  \eat{
Recent advances in molecular sequencing technology have ushered in the era of metagenomics, whereby whole communities of organisms are sequenced rather than individual isolates.
Metagenomic sequencing projects are typically done with high-throughput shotgun sequencing technology, giving a collection of reads in the 100 to 600 nucleotide range with no signal of which gene or even which organism the reads came from.
This abundance of metagenomic short reads raises a very difficult question for bioinformaticians: how to place these short reads into previously-characterized diversity? 
Equally as important, how do we assess confidence of these placements?
In this paper we present "\pplacer", which phylogenetically places short reads in a user-supplied reference gene tree.
What differentiates \pplacer\ from other related approaches is it fixes the reference tree with respect to both topology and branch length.
This has three advantages:
% question: how to talk about speed and PP?
First, fixing the tree in this way allows us to calculate the posterior probability of the placement by direct numerical integration; in doing so it gives us a statistically rigorous way to evaluate placement.
Second, our simulation results indicate that fixing the tree improves accuracy.
Third, fixing the reference tree allows the algorithm to run very quickly, at a rate of about 1000 reads an hour on an 80-taxon reference tree.



Furthermore, these constraints make it possible for the phylogenetic algorithm to run very quickly, such that a single processor running \pplacer\ can place about one thousand reads an hour into a reference tree on 80 taxa under the maximum-likelihood criterion.
%In maximum-likelihood mode, it finds the edge, edge cut, and pendant edge length which maximize 
%can also determine placements based on the "likelihood weight distribution" in a similar way but in a maximum likelihood context.
\Pplacer can also be run in a slower but more statistically rigorous Bayesian approach, where various possible phylogenetic positions of the read are evaluated according to normalized posterior probability; because we are fixing a reference tree, we can perform direct numerical integration over the likelihood function to obtain confidence estimates rather than resorting to Markov chain Monte-Carlo procedures. 
% Pplacer is a stand-alone program which allows the user to supply a reference alignment and tree; it can be used via a simple command line interface or as part of a pipeline. % robs-- do you like this sentence?
We have also implemented large-scale short read simulation which demonstrates the effectiveness of our method across 829 of genes with differing levels of divergence.
% Such simulations have also given us a new perspective on what phylogenetic placement scores mean, namely that posterior probability being spread over a number of locations can indicate global rather than local uncertainty.
}



\section{post}
% \Pplacer\ takes advantage of the special structure of the problem, caching data to achieve a very significant savings in computation.
% Furthermore, because the complexity of the algorithm scales linearly with the size of reference tree and the number of reads, the advantages of \pplacer\ will become especially apparent in the future as the number of reference sequences and the environmental sequence databases continue to increase in size.
% \Pplacer\ can calculate the posterior probability of a placement given the fixed reference tree, as well as the ``likelihood weight ratio,'' \cite{vonMeringEaQuantitative08} i.e. the normalized ML likelihood values where one optimizes only the pendant branch length and the attachment location on the chosen branch.
% We will refer to each of these as ``confidence scores.''




% we don't have to reduce to names
Although taxonomic classifications can be extracted from the placement into the reference tree, the placements themselves can be used in downstream analyses.
Using the placements directly gives more information than a taxonomic name can convey.
For example, a placement at an internal edge of the tree says that although the query sequence may fit in a given clade, it is not any one of the individual sequences in the clade.
This can indicate when something truly new is seen.
This difference becomes quite important in cases, such as for eukaryotic phytoplanka, when the reference tree is sparse.



%The main focus of our simulation study is a large-scale simulation using \ncogs\ alignments downloaded from the COG database \cite{tatusov1997genomic}. 
%These alignments were manually edited to eliminate very short reference sequences and to trim the ends of the alignments.  
%The main focus of the simulation study was to evaluate the \pplacer\ placements and confidence scores, and to address the role of phylogenetic signal in this type of analysis.  
%We also did two single gene simulations for detailed analysis, one using amino acids and the other using nucleotides.
%All simulations were done using the same pipeline consisting of a collection of \texttt{python} and \texttt{ocaml} code which is available upon request.





\subsection*{Table \tabOSC\ - Accuracy comparison on oxidosqualene cyclase: read length mean of 34aa}

\begin{tabular}{r|ccc}
error	& ML fixed ref	& ML flex ref	& PP \\ 
\hline
0	& 185	& 184	& 182	 \\ 
1	& 108	& 108	& 112	 \\ 
2	& 31	& 29	& 29	 \\ 
3	& 17	& 19	& 17	 \\ 
4	& 5	& 6	& 7	 \\ 
5	& 5	& 5	& 4	 \\ 
6	& 1	& 1	& 1	 \\ 
7	& 0	& 0	& 0	 \\ 
8	& 0	& 0	& 0	 \\ 
9	& 0	& 0	& 0	 \\ 
10	& 1	& 1	& 1	 \\ 
\end{tabular}

\hspace{0.5cm}

Results of the oxidosqualene cyclase gene simulation as described in the text. 
The amino acid lengths of the fragments were drawn from a normal distribution of mean 34 and standard deviation 5.
The far left column shows the error, and the other columns show the frequency of the error for the different placement methods. 
``ML fixed ref'' means maximum likelihood (ML) placement with the reference tree fixed with respect to branch length and topology,
``ML flex ref'' means ML placement where all of the branch lengths are allowed to vary, and
``PP'' is short for posterior probability.
For example, the first entry of the ``ML fixed ref'' column signifies that out of the 353 simulated fragments that satisfied our HMMER E-value cutoff, 185 reads were placed in exactly the correct location.
This table and the next show essentially equivalent performance of all three strategies in terms of the accuracy of their top placement.



\newpage

\subsection*{Table \tabActin\ - Accuracy comparison on actin}

\hspace{0.5cm}

An equivalent simulation to that in Table~\tabOSC, except a nucleotide alignment of actin was used.
Read lengths normally distributed with mean 250 and standard deviation of 60 nucleotides.
Again, we can see little significant difference between the three methods in terms of the accuracy of their top placements.

\begin{tabular}{r|ccc}
error	& ML fixed ref	& ML flex ref	& PP \\ 
\hline
0	& 212	& 211	& 212	 \\ 
1	& 118	& 122	& 139	 \\ 
2	& 92	& 95	& 84	 \\ 
3	& 56	& 55	& 52	 \\ 
4	& 43	& 37	& 44	 \\ 
5	& 34	& 30	& 28	 \\ 
6	& 24	& 26	& 25	 \\ 
7	& 26	& 30	& 23	 \\ 
8	& 31	& 25	& 30	 \\ 
9	& 17	& 20	& 16	 \\ 
10	& 15	& 13	& 15	 \\ 
11	& 7	& 8	& 6	 \\ 
12	& 13	& 14	& 14	 \\ 
13	& 7	& 8	& 8	 \\ 
14	& 12	& 12	& 10	 \\ 
15	& 1	& 1	& 2	 \\ 
16	& 2	& 2	& 2	 \\ 
17	& 3	& 4	& 3	 \\ 
18	& 0	& 0	& 0	 \\ 
19	& 0	& 0	& 0	 \\ 
20	& 1	& 1	& 1	 \\ 
\end{tabular}





% This metric has the advantage of simplicity and generality, however, it is presented here with certain caveats.
% \Pplacer\ does not use any branch length information in the tree, which means that an error traversing a collection of long edges will score the same as error traversing the same number of short edges; thus well-sampled parts of the tree will be scored more strictly than sparsely sampled parts of the tree.
% Information about where to place the fragment is much better in well-sampled regions and algorithms should be expected to perform with higher accuracy.
% An alternative approach is to sum the branch lengths on the path from the correct to the placed location, but in the Bayesian setting integration occurs over a variety of branch lengths, complicating scoring with respect to branch length. 
% We also admit that our scoring function is not explicitly taxonomic, such that an error of a certain size under our metric may represent simply a species-level mis-assignment or a super-kingdom mis-assignment.
% However, reference trees may contain paralogous genes, and we are specifically interested in which copy a given fragment represents. 
% We are not aware of a natural score to compare a placement that is not in the correct phylum but does represent the correct copy, versus a placement that is the correct phylum but not the correct copy.
% Our simple metric allows us to use the phylogenetic information available for practical use without having to solve these ambiguities. 


\subsubsection*{Comparative simulations}
We also performed simulations to understand how well our method performs compared to methods that allow the branch lengths of the reference tree to vary \cite{monierEaLargeViruses08, vonMeringEaQuantitative08}. 
Because neither ``phylomapping'' nor ``MLTreeMap'' implementations were freely available, we wrote wrapper scripts to perform the equivalent analysis with the PHYML package \cite{guindonGascuelPHYML03}.
Such an approach (which requires a considerable amount of re-calculation on the reference tree) is necessarily much slower. 
Thus we could not perform the \ncogs-gene simulation described previously, and settled on two genes for comparative analysis: a protein alignment of oxidosqualene cyclase (OSC), and a nucleotide alignment of actin.  
OSC was chosen for its use in metagenomics because it is a single copy gene involved in biosynthesis of sterols, a class of lipids that are synapomorphic to all eukaryotes; we find it to recapitulate eukaryotic phylogeny as determined with our multi-gene analysis.  
Actin was chosen because it is a gene also found in all eukaryotes and is well represented in metagenomic databases.
Reference sequences for each gene were obtained from GenBank or from our in-house database.
Minimal differences between the overall accuracy of the three placement methods were detected (Tables~\tabOSC\ and \tabActin). 
The only differences were the types of confidence scores provided and the increased speed of \pplacer.
We also used OSC to ask questions about how fragment length and fragment position relative to the reference alignment determine placement accuracy (supplemental Figure~\sfiglocation), and if HMMER E-value can be used as a predictor of placement accuracy (supplemental Figure~\sfigevalue).

\subsection*{Table~\tabcomparison\ - Comparison of \pplacer\ to previous software}
\begin{tabular}{l|cccccc}
software                                          &  complexity  &  available     &  ML          &  PP          \\
\hline
\pplacer\                                         &  linear      &  \checkmark    &  \checkmark  &  \checkmark  \\
Phylomapping  \cite{monierEaLargeViruses08}       &  quadratic   &                &  \checkmark  &              \\
MLTreeMap     \cite{vonMeringEaQuantitative08}    &  quadratic   &  limited web   &  \checkmark  &              \\
SAP \cite{munchEaBarcoding08} \cite{munchEaSAP08} &  cubic/hard  &  \checkmark    &              &  \checkmark  \\
MEGAN         \cite{husonEaMEGAN07}               &  linear      &  \checkmark    &              &              \\
CARMA         \cite{krause2008pcs}                &  cubic       &  \checkmark    &              &              \\
\end{tabular}


\hspace{0.5cm}

Comparison of metagenome classification methods.
Notes: 
The web implementation of MLTreeMap \cite{vonMeringEaQuantitative08} is limited in that it is tied to core bacterial genes and that it and allows only one read to be placed at a time.
SAP uses neighbor-joining (cubic complexity) or Bayesian MCMC iteration, which takes about an hour with 50 reference sequences by the authors' estimate \cite{munchEaSAP08}.
\Pplacer\ and SAP differ in the posterior probability that they calculate: \pplacer\ conditions on the reference tree in terms of topology and branch length, while SAP does not.
\newpage




\subsection*{Figure~\figflow: \pplacer\ flowchart}
\bmcNoSumbmit{\includegraphics[width= 5.5in]{PplaceFlow_figure.pdf}}

After preparing a reference tree and a profile HMM from the reference alignment, a complete \pplacer\ run consists of three steps.
First, a search through the metagenome database using a \texttt{python} wrapper around the \texttt{hmmsearch} program of the HMMER \cite{eddyProfileHMMs98} package finds reads homologous to the reference alignment.
The result of this step is a collection of reads for the gene of interest that have been aligned to the reference alignment.
Second, these aligned reads along with the reference tree and alignment are fed into \texttt{pplacer}, which evaluates all placement locations for each read on a phylogenetic tree.
Third, these placements can visualized in a number of different ways from the self-contained \texttt{.place} file.




% using pplacer
\robs{do you think we need this paragraph? seems like more appropriate for the manual}
To use \pplacer\ with metagenomic data, the metagenomic reads of the gene of interest need to be identified in the metagenome database and aligned to the reference alignment.
To accomplish this in a single step, HMMER \cite{eddyProfileHMMs98} is used to search the database with a profile hidden Markov model (HMM), which is generated from the reference alignment.
The profile HMM, which is a statistical model of the reference alignment, is used to search the read database and align the recruited reads to the reference alignment.
The file of aligned fragments recruited by HMMER can then be run in \pplacer\ along with the reference tree and the reference alignment.
% (Figure~\figflow).
Although phylogenetic placement is more demanding than other analysis methods to automate, \pplacer\ is designed such that the reference information can easily be isolated from the rest of the data, and as described below \placeviz\ can separate and merge .place files to ease parallization and sample separation.




However, measures such as these that describe confidence on an edge-by-edge basis can have difficulty distinguishing between local and global uncertainty.
Although there may be considerable uncertainty as to the best edge among an given set of edges, the optimal placement location can be quite certain if the attachment locations are close to each other on those edges.
This problem manifests itself in that placements landing in a region of the tree with many similar sequences will often be assigned low likelihood weight ratio or posterior probabilities.
These low confidence scores can skew downstream analyses if uncertain ones are removed from the analysis.

We acknowledge that the reference tree may in fact be wrong for a given taxon, and so our error metric will be skewed for that taxon.
However, if one believes the results of phylogeny at all, it is a reasonable and non-trivial question to ask if one can recover the results of a phylogenetic analysis with full-length sequences using short fragments as we have done here.

The identification of new higher level taxonomic groups in environmental sequence samples poses a difficult challenge for taxonomic identification methods.  
Simple sequence similarity searches do not enable this type of discovery, as a query sequence will either be similar to a collection of organisms, or will not be similar to any of them.
Phylogenetic analysis, however, provides the option of placing the unknown environmental sequences at ancestral nodes in the tree, indicating a potentially new group of organisms.
% Accurate placement at higher taxonomic levels is difficult, especially when the closest relative is distant phylogenetically such as with new higher taxonomic levels.

% cut..
We emphasize that the focus of this simulation was on the relationship between the edge-level confidence in the tree and the accuracy as measured on an edge-by-edge basis. 
It would have been possible to score simulation results using the distance along the tree and measure uncertainty via the EDPL, however the result of such a simulation would have been tautological: if placements were spread between distant locations in the tree, then by necessity they can't all be close to the correct location.




